Design of Soft, Modular Appendages for a Bio-inspired Multi-Legged Terrestrial Robot

Soft robots have the ability to adapt to their environment, which makes them suitable for use in disaster areas and agricultural fields, where their mobility is constrained by complex terrain. One of the main challenges in developing soft terrestrial robots is that the robot must be soft enough to adapt to its environment, but also rigid enough to exert the required force on the ground to locomote. In this paper, we report a pneumatically driven, soft modular appendage made of silicone for a terrestrial robot capable of generating specific mechanical movement to locomote and transport loads in the desired direction. This two-segmented soft appendage uses actuation in between the joint and the lower segment of the appendage to ensure adequate rigidity to exert the required force to locomote. A prototype of a soft-rigid-bodied tethered physical robot was developed and two sets of experiments were carried out in both air and underwater environments to assess its performance. The experimental results address the effectiveness of the soft appendage to generate adequate force to navigate through various environments and our design method offers a simple, low-cost, and efficient way to develop terradynamically capable soft appendages that can be used in a variety of locomotion applications.

==> bibtex.tex <==
\begin{thebibliography}
\bibitem{chen2021legless}
R.~Chen, Z.~Yuan, J.~Guo, L.~Bai, X.~Zhu, F.~Liu, H.~Pu, L.~Xin, Y.~Peng,
  J.~Luo, {\em et~al.}, ``Legless soft robots capable of rapid, continuous, and
  steered jumping,'' {\em Nature Communications}, vol.~12, no.~1, pp.~1--12,
  2021.

\bibitem{lu2018bioinspired}
H.~Lu, M.~Zhang, Y.~Yang, Q.~Huang, T.~Fukuda, Z.~Wang, and Y.~Shen, ``A
  bioinspired multilegged soft millirobot that functions in both dry and wet
  conditions,'' {\em Nature communications}, vol.~9, no.~1, pp.~1--7, 2018.

\bibitem{huang2018chasing}
X.~Huang, K.~Kumar, M.~K. Jawed, A.~M. Nasab, Z.~Ye, W.~Shan, and C.~Majidi,
  ``Chasing biomimetic locomotion speeds: Creating untethered soft robots with
  shape memory alloy actuators,'' {\em Science Robotics}, vol.~3, no.~25,
  p.~eaau7557, 2018.

\bibitem{mao2022ultrafast}
G.~Mao, D.~Schiller, D.~Danninger, B.~Hailegnaw, F.~Hartmann, T.~Stockinger,
  M.~Drack, N.~Arnold, and M.~Kaltenbrunner, ``Ultrafast small-scale soft
  electromagnetic robots,'' {\em Nature Communications}, vol.~13, no.~1,
  pp.~1--11, 2022.

\bibitem{wu2019insect}
Y.~Wu, J.~K. Yim, J.~Liang, Z.~Shao, M.~Qi, J.~Zhong, Z.~Luo, X.~Yan, M.~Zhang,
  X.~Wang, {\em et~al.}, ``Insect-scale fast moving and ultrarobust soft
  robot,'' {\em Science Robotics}, vol.~4, no.~32, p.~eaax1594, 2019.

\bibitem{huang2022insect}
H.~Huang, Y.~Feng, X.~Yang, L.~Yang, and Y.~Shen, ``An insect-inspired
  terrains-adaptive soft millirobot with multimodal locomotion and
  transportation capability,'' {\em Micromachines}, vol.~13, no.~10, p.~1578,
  2022.

\bibitem{lin2013soft}
H.-T. Lin, G.~Leisk, and B.~Trimmer, ``Soft robots in space: a perspective for
  soft robotics,'' {\em Acta Futura}, vol.~6, pp.~69--79, 2013.

\bibitem{shah2021soft}
D.~S. Shah, J.~P. Powers, L.~G. Tilton, S.~Kriegman, J.~Bongard, and
  R.~Kramer-Bottiglio, ``A soft robot that adapts to environments through shape
  change,'' {\em Nature Machine Intelligence}, vol.~3, no.~1, pp.~51--59, 2021.

\bibitem{ozkan2021self}
Y.~Ozkan-Aydin and D.~I. Goldman, ``Self-reconfigurable multilegged robot
  swarms collectively accomplish challenging terradynamic tasks,'' {\em Science
  Robotics}, vol.~6, no.~56, p.~eabf1628, 2021.

\bibitem{waynelovich2016versatile}
J.~Waynelovich, T.~Frey, A.~Baljon, and P.~Salamon, ``Versatile and dexterous
  soft robotic leg system for untethered operations,'' {\em Soft Robotics},
  vol.~3, no.~2, pp.~64--70, 2016.

\bibitem{tang2020leveraging}
Y.~Tang, Y.~Chi, J.~Sun, T.-H. Huang, O.~H. Maghsoudi, A.~Spence, J.~Zhao,
  H.~Su, and J.~Yin, ``Leveraging elastic instabilities for amplified
  performance: Spine-inspired high-speed and high-force soft robots,'' {\em
  Science advances}, vol.~6, no.~19, p.~eaaz6912, 2020.

\bibitem{guo2017design}
H.~Guo, J.~Zhang, T.~Wang, Y.~Li, J.~Hong, and Y.~Li, ``Design and control of
  an inchworm-inspired soft robot with omega-arching locomotion,'' in {\em 2017
  IEEE International Conference on Robotics and Automation (ICRA)},
  pp.~4154--4159, IEEE, 2017.

\bibitem{calisti2017fundamentals}
M.~Calisti, G.~Picardi, and C.~Laschi, ``Fundamentals of soft robot
  locomotion,'' {\em Journal of The Royal Society Interface}, vol.~14, no.~130,
  p.~20170101, 2017.

\bibitem{kim2013soft}
S.~Kim, C.~Laschi, and B.~Trimmer, ``Soft robotics: a bioinspired evolution in
  robotics,'' {\em Trends in biotechnology}, vol.~31, no.~5, pp.~287--294,
  2013.

\bibitem{xia2021legged}
B.~Xia, J.~Fu, H.~Zhu, Z.~Song, Y.~Jiang, and H.~Lipson, ``A legged soft robot
  platform for dynamic locomotion,'' in {\em 2021 IEEE International Conference
  on Robotics and Automation (ICRA)}, pp.~11812--11819, IEEE, 2021.

\bibitem{mueller2019voxelated}
J.~Mueller, M.~Skylar-Scott, C.~Visser, and J.~Lewis, ``Voxelated soft matter
  via multimaterial multinozzle 3d printing,'' {\em Nature}, 2019.

\bibitem{rus2015design}
D.~Rus and M.~T. Tolley, ``Design, fabrication and control of soft robots,''
  {\em Nature}, vol.~521, no.~7553, pp.~467--475, 2015.

\bibitem{Yim2007}
M.~Yim, W.-m. Shen, B.~Salemi, D.~Rus, M.~Moll, H.~Lipson, E.~Klavins, and
  G.~S. Chirikjian, ``Modular self-reconfigurable robot systems [grand
  challenges of robotics],'' {\em IEEE Robotics \& Automation Magazine},
  vol.~14, no.~1, pp.~43--52, 2007.

\bibitem{MOUBARAK20121648}
P.~Moubarak and P.~Ben-Tzvi, ``Modular and reconfigurable mobile robotics,''
  {\em Robotics and Autonomous Systems}, vol.~60, no.~12, pp.~1648--1663, 2012.

\bibitem{Post2021}
M.~A. Post, X.-T. Yan, and P.~Letier, ``Modularity for the future in space
  robotics: A review,'' {\em Acta Astronautica}, vol.~189, pp.~530--547, 2021.

\bibitem{drotman20173d}
D.~Drotman, S.~Jadhav, M.~Karimi, P.~de~Zonia, and M.~T. Tolley, ``3d printed
  soft actuators for a legged robot capable of navigating unstructured
  terrain,'' in {\em 2017 IEEE International Conference on Robotics and
  Automation (ICRA)}, pp.~5532--5538, IEEE, 2017.

\bibitem{OzkanAydin_Centipede}
Y.~Ozkan-Aydin, B.~Chong, E.~Aydin, and D.~I. Goldman, ``A systematic approach
  to creating terrain-capable hybrid soft/hard myriapod robots,'' in {\em 2020
  3rd IEEE International Conference on Soft Robotics (RoboSoft)}, pp.~156--163,
  2020.

\bibitem{shepherd2011multigait}
R.~F. Shepherd, F.~Ilievski, W.~Choi, S.~A. Morin, A.~A. Stokes, A.~D. Mazzeo,
  X.~Chen, M.~Wang, and G.~M. Whitesides, ``Multigait soft robot,'' {\em
  Proceedings of the national academy of sciences}, vol.~108, no.~51,
  pp.~20400--20403, 2011.

\bibitem{baines2022multi}
R.~Baines, S.~K. Patiballa, J.~Booth, L.~Ramirez, T.~Sipple, A.~Garcia,
  F.~Fish, and R.~Kramer-Bottiglio, ``Multi-environment robotic transitions
  through adaptive morphogenesis,'' {\em Nature}, vol.~610, no.~7931,
  pp.~283--289, 2022.

\bibitem{venkiteswaran2019bio}
V.~K. Venkiteswaran, L.~F.~P. Samaniego, J.~Sikorski, and S.~Misra,
  ``Bio-inspired terrestrial motion of magnetic soft millirobots,'' {\em IEEE
  Robotics and automation letters}, vol.~4, no.~2, pp.~1753--1759, 2019.

\bibitem{kalin2020design}
M.~A.~I. Kal{\i}n, C.~Ayg{\"u}l, A.~T{\"u}rkmen,
  J.~Kwiczak-Yi{\u{g}}itba{\c{s}}{\i}, B.~Baytekin, and O.~{\"O}zcan, ``Design,
  fabrication, and locomotion analysis of an untethered miniature soft
  quadruped, squad,'' {\em IEEE Robotics and Automation Letters}, vol.~5,
  no.~3, pp.~3854--3860, 2020.

\bibitem{xavier2021finite}
M.~S. Xavier, A.~J. Fleming, and Y.~K. Yong, ``Finite element modeling of soft
  fluidic actuators: Overview and recent developments,'' {\em Advanced
  Intelligent Systems}, vol.~3, no.~2, p.~2000187, 2021.

\bibitem{hwang2015pneumatic}
Y.~Hwang, O.~H. Paydar, and R.~N. Candler, ``Pneumatic microfinger with balloon
  fins for linear motion using 3d printed molds,'' {\em Sensors and Actuators
  A: Physical}, vol.~234, pp.~65--71, 2015.

\bibitem{konishi2001thin}
S.~Konishi, F.~Kawai, and P.~Cusin, ``Thin flexible end-effector using
  pneumatic balloon actuator,'' {\em Sensors and Actuators A: Physical},
  vol.~89, no.~1-2, pp.~28--35, 2001.

\bibitem{Hildebrand}
M.~Hildebrand, ``Symmetrical gaits of primates,'' {\em American Journal of
  Physical Anthropology}, vol.~26, no.~2, pp.~119--130, 1967.

\end{thebibliography}
